Electrical Vehicle Fleet Routing Accounting for Dynamic Battery Degradation

The increasing uptake of electrical vehicles (EVs) has increased the awareness of battery degradation costs and how they can be minimized. However, from a planning perspective it is difficult to integrate battery degradation models into existing route planning models and to assess how policies that aim at reducing battery degradation affect route planning costs and degradation across the fleet. In this paper, a simple transportation vehicle routing problem (VRP) is formulated as a mixed-integer nonlinear problem (MINLP), with a modification that allows monitoring the maximum and minimum depth-of-discharge (DoD) of the entire fleet. This allows us to measure the battery health degradation during the online optimization process. The results show that accounting for the impact of different route characteristics on battery degradation can have an impact on the route planning of the entire fleet as well as the battery degradation for all vehicles. The latter is achieved by forcing vehicles to adapt to certain DoD boundaries in the long term.

==> Paper_Planning.tex <==
Plan A: something Jeppe sends...
Plan B: doesn't work...
Plan C: don't get anything (tap into him anyways). 
  - Simple model ("simple" routes (same vehicle  versus some type of
  
Plan D: bus 1 goes through deep cycles, bus 2 does not; you need to cycle.
Two main metrics: Total energy consumption over the day, and worst battery w.r.t. degradation. 
Constraints: fulfill customer request (logistic deliveries, including buses, AV taxis (more random but anyway), etc.) 

Also, 

Nice figures. 












Plan A: something Jeppe sends...
Plan B: doesn't work...
Plan C: don't get anything (tap into him anyways). 
  - Simple model ("simple" routes (same vehicle  versus some type of
  
Plan D: bus 1 goes through deep cycles, bus 2 does not; you need to cycle.
Two main metrics: Total energy consumption over the day, and worst battery w.r.t. degradation. 
Constraints: fulfill customer request (logistic deliveries, including buses, AV taxis (more random but anyway), etc.) 

Also, 

Nice figures. 


  
  >> driving style as future work

Then: 
"Demand for plug-in electric vehicles across segments in the future vehicle market" \cite{Jensen_Rich_2021}. 




% Electric cars, which accounted for 2.6% of global car sales and about 1% of global car stock in 2019, registered a 40% year-on-year increase. As technological progress in the electrification of two/three-wheelers, buses, and trucks advances and the market for them grows, electric vehicles are expanding significantly. Ambitious policy announcements have been critical in stimulating the electric-vehicle rollout in major vehicle markets in recent years. In 2019, indications of a continuing shift from direct subsidies to policy approaches that rely more on regulatory and other structural measures – including zero-emission vehicles mandates and fuel economy standards – have set clear, long-term signals to the auto industry and consumers that support the transition in an economically sustainable manner for governments. 
% \cite{IEA_Global_EV_2020}.
% As the electrification of transport gains momentum, some cities are facilitating the integration of EVs and renewable power supply, installing EV charging stations or public transport infrastructure that relies on renewable electricity \cite{REN21_2020}, and companies are investing more in it. Nerve Smart Systems, OK, TopCharge and HEART...
